Fine-grained complexity of the list homomorphism problem: feedback vertex set and cutwidth

For graphs $G,H$, a homomorphism from $G$ to $H$ is an edge-preserving mapping from $V(G)$ to $V(H)$. In the list homomorphism problem, denoted by \textsc{LHom}($H$), we are given a graph $G$ and lists $L: V(G) \to 2^{V(H)}$, and we ask for a homomorphism from $G$ to $H$ which additionally respects the lists $L$. Very recently Okrasa, Piecyk, and Rz\k{a}\.zewski [ESA 2020] defined an invariant $i^*(H)$ and proved that under the SETH $\mathcal{O}^*\left (i^*(H)^{\textrm{tw}(G)}\right)$ is the tight complexity bound for \textsc{LHom}($H$), parameterized by the treewidth $\textrm{tw}(G)$ of the instance graph $G$. We study the complexity of the problem under dirretent parameterizations. As the first result, we show that $i^*(H)$ is also the right complexity base if the parameter is the size of a minimum feedback vertex set of $G$. Then we turn our attention to a parameterization by the cutwidth $\textrm{ctw}(G)$ of $G$. Jansen and Nederlof~[ESA 2018] showed that \textsc{List $k$-Coloring} (i.e., \textsc{LHom}($K_k$)) can be solved in time $\mathcal{O}^*\left (c^{\textrm{ctw}(G)}\right)$ where $c$ does not depend on $k$. Jansen asked if this behavior extends to graph homomorphisms. As the main result of the paper, we answer the question in the negative. We define a new graph invariant $mim^*(H)$ and prove that \textsc{LHom}($H$) problem cannot be solved in time $\mathcal{O}^*\left ((mim^*(H)-\varepsilon)^{\textrm{ctw}(G)}\right)$ for any $\varepsilon >0$, unless the SETH fails. This implies that there is no $c$, such that for every odd cycle the non-list version of the problem can be solved in time $\mathcal{O}^*\left (c^{\textrm{ctw}(G)} \right)$. Finally, we generalize the algorithm of Jansen and Nederlof, so that it can be used to solve \textsc{LHom}($H$) for every graph $H$; its complexity depends on $\textrm{ctw}(G)$ and another invariant of $H$, which is constant for cliques.

==> intro-old.tex <==
One of the most classical graph problems is $k\coloring$ in which for a given graph $G$ we have to decide whether it is possible to properly color the vertices of $G$ with $k$ colors. A graph homomorphism problem $\homo H$ is a natural extension of coloring. For a fixed graph $H$ in $\homo H$ we have to decide if for a given graph $G$ there exists a mapping $\vphi: V(G) \to V(H)$ such that for every $uv \in E(G)$ it holds $\vphi(u)\vphi(v) \in E(H)$. Note that for $H \simeq K_k$ the $\homo H$ problem is equivalent to $k\coloring$.

It is well known that the $k\coloring$ problem is polynomial-time solvable for $k<3$ and NP-complete otherwise. In $\homo H$ we can distinguish two ``easy'' cases. First, if $H$ contains a vertex $v$ with a loop, then every instance $G$ of $\homo H$ is a \textsc{Yes}-instance since we can map every vertex of $G$ to the vertex $v$. In irreflexive case (if $H$ does not contain a loop),  Hell and Ne\v{s}et\v{r}il \cite{DBLP:journals/jct/HellN90} provided a dichotomy theorem for $\homo H$ -- it is polynomial-time solvable if $H$ is bipartite and NP-complete otherwise.

In this paper we consider a list version of the homomorphism problem, $\lhomo H$, in which every instance consists of a graph $G$ and lists $L: V(G) \to 2^{V(H)}$, and we have to decide whether there exists a homomorphism from $G$ to $H$ that additionally respects lists $L$. Note that, even if $H$ contains a loop, $\lhomo H$ might not be polynomial-time solvable since we might not be able to map all vertices to a vertex with a loop because of the lists. Feder and Hell \cite{FEDER1998236} proved that for reflexive $H$ (i.e., every vertex of $H$ has a loop) $\lhomo H$ is polynomial-time solvable if $H$ is an interval graph and NP-complete otherwise. For bipartite Feder, Hell, and Huang \cite{DBLP:journals/combinatorica/FederHH99} showed that $\lhomo H$ is  polynomial-time solvable if $H$ is a complement of a circular-arc graph and NP-complete otherwise. Finally, for any $H$ (with loops allowed) they provided full classification of $\lhomo H$ -- it is  polynomial-time solvable if $H$ is a bi-arc graph and NP-complete otherwise \cite{DBLP:journals/jgt/FederHH03}.

Nowadays, it is very popular to study the complexity of the problems more carefully. In particular, the aim is to find out how actually hard are the problems, that we already know to be NP-hard, if we restrict to some specific graph classes. The research is done in both directions, improving algorithms and lower bounds, so that we get a tight complexity.

In order to prove better lower bounds, we need a stronger assumption than $P\neq NP$. The common assumption is the conjecture called \emph{the Strong Exponential Time Hypothesis} (SETH) that states the complexity of the following problem. In the \textsc{CNF-Sat} we are given a logic formula in conjunctional normal form, with $n$ variables and $m$ clauses. We have to decide whether there exists a truth assignment of the variables satisfying the formula. Obviously, there is a trivial algorithm that solves \textsc{CNF-Sat} in time $2^n \cdot (n\cdot m)^{\Oh(1)}$. While $P\neq NP$ implies that \textsc{CNF-Sat} cannot be solved in polynomial-time, the SETH gives us tight lower bound. 

\begin{conjecture}[ETH]
There exists $\delta > 0$, such that \textsc{3-Sat} with $n$ variables cannot be solved in time $2^{\delta \cdot n} \cdot n^{\Oh(1)}$.
\end{conjecture}
\begin{conjecture}[SETH]
\textsc{CNF-Sat} with $n$ variables and $m$ clauses cannot be solved in time $(2-\eps)^n \cdot m^{\Oh(1)}$ for any $\eps>0$.
\end{conjecture}

In the other direction, i.e., improving algorithms while restricting to special classes, it is common to consider graphs with bounded certain parameters, like for example the treewidth. The idea of restricting to graphs with bounded treewidth is based on the fact that many problems are easy on trees, since we can use dynamic programming. If a graph $G$ is given along with a tree decomposition of width $\tw{G}$, then we can solve the problem quite efficiently using dynamic programming on the tree decomposition. Another parameter that is also based on the fact that trees are ``easy'' is the size of a minimum \emph{feedback vertex set} (the set of vertices in $G$ such that every cycle in $G$ contains at least one vertex from that set) denoted by $\fvs{G}$. If we assume that $G$ is given along with a feedback vertex set $F$ of size $\fvs{G}$, then we can guess the solution on $F$ and then solve the problem on the rest of the graph, which by the definition is a forest and thus is easy. 

One of the examples of results in the complexity parametrized by treewidth or feedback vertex set is the following theorem for the $k\coloring$ problem, by Lokshtanov, Marx, and Saurabh \cite{DBLP:conf/soda/LokshtanovMS11a}.

\begin{theorem}[Lokshtanov, Marx, Saurabh~\cite{DBLP:conf/soda/LokshtanovMS11a}]\label{thm:LMS}
Let $k \geq 3$. Then the $k \coloring$ on an instance $G$
\begin{enumerate}[a)]
%\item can be solved in time $k^{\tw{G}}\cdot n^{\Oh(1)}$, provided that $G$ is given along with a tree decomposition $\tw{G}$,\prz{algorytmiczna część tego to powszechnie znana rzecz, nie powinna sie znaleźć w tym twierdzeniu}
\item cannot be solved in time $(k-\epsilon)^{\pw{G}} \cdot |V(G)|^{\Oh(1)}$ for any $\eps>0$, unless the SETH fails,
\item cannot be solved in time $(k-\epsilon)^{\fvs{G}} \cdot |V(G)|^{\Oh(1)}$ for any $\eps>0$, unless the SETH fails.
\end{enumerate}
\end{theorem}

It is well known that $\tw{G} \leq \fvs{G}+1$ and $\tw{G}\leq\pw{G}$, where $\pw{G}$ is incomparable with $\fvs{G}$. Moreover, if $G$ is given with a feedback vertex set of size $\fvs{G}$, then in polynomial-time we can construct a tree decompositon of $G$ of width $\fvs{G}+1$. Thus the mentioned upper bound for treewidth implies a similar upper bound for feedback vertex set and pathwidth and each of the lower bounds for feedback vertex set and pathwidth implies the lower bound for treewidth.

The natural question is to prove similar bounds for the $\lhomo H$ problem. This was done for treewidth and pathwidth in \cite{LhomoTreewidth}, for a certain invariant $i^*(H)$.

\begin{theorem}[Okrasa, Piecyk, Rzążewski \cite{LhomoTreewidth}]
Let $H$ be a connected, non-bi-arc graph.
\begin{enumerate}[a)]
\item Even if $H$ is given in the input, every instance $(G,L)$ of  $\lhomo H$ can be solved in time $i^*(H)^{\tw{G}}\cdot (|V(G)| \cdot |V(H)|)^{\Oh(1)}$, provided that $G$ is given along with a tree decomposition of width $\tw{G}$.
\item Even if $H$ is fixed, there is no algorithm that solves every instance $(G,L)$ of $\lhomo H$ in time $(i^*(H)-\eps)^{\pw{G}}\cdot (|V(G)| \cdot |V(H)|)^{\Oh(1)}$ for any $\eps>0$, unless the SETH fails.
\end{enumerate}
\end{theorem}

In this paper we show the tight complexity of the $\lhomo H$ parameterized by $\fvs{G}$. 

\begin{theorem} \label{thm:main}
Let $H$ be a connected, non-bi-arc graph.
\begin{enumerate}[a)]
\item Even if $H$ is given in the input, every instance $(G,L)$ of  $\lhomo H$ can be solved in time $i^*(H)^{\fvs{G}}\cdot (|V(G)| \cdot |V(H)|)^{\Oh(1)}$, provided that $G$ is given along with a feedback vertex set of size $\fvs{G}$.
\item Even if $H$ is fixed, there is no algorithm that solves every instance $(G,L)$ of $\lhomo H$ in time $(i^*(H)-\eps)^{\fvs{G}}\cdot (|V(G)| \cdot |V(H)|)^{\Oh(1)}$ for any $\eps>0$, unless the SETH fails.
\end{enumerate}
\end{theorem}

Then bla bla bla cutwidth.

\begin{restatable}{theorem}{mainctwlhomo}
%\begin{theorem}
\label{thm:main-ctw-list-hard}
Let $\mathcal{H}$ be the class of connected non-bi-arc graphs.
Let $g$ be a positive integer, and let $\mathcal{C}_g$ be the class of subcubic bipartite graphs $G$ with girth at least $g$, such that vertices of degree $3$ in $G$ are at distance at least $g$.
\begin{enumerate}[a)]
\item For every $H \in \mathcal{H}$, there is no algorithm that solves every instance $(G,L)$ of  $\lhomo H$, where $G \in \mathcal{C}_g$, in time $(mim^*(H)-\epsilon)^{\ctw{G}} \cdot |V(G)|^{\Oh(1)}$ for any $\epsilon > 0$, unless the SETH fails,
\item There exists a universal constant $0<\delta<1$, such that for every $H \in \mathcal{H}$, there is no algorithm that solves every instance $(G,L)$ of $\lhomo H$, where $G \in \mathcal{C}_g$, in time $mim^*(H)^{\delta \cdot \ctw{G}} \cdot |V(G)|^{\Oh(1)}$, unless the ETH fails.
\end{enumerate}
%\end{theorem}
\end{restatable}

For a graph $F$, we say that $G$ is $F$-free if it does not contain $F$ as an induced subgraph.
We observe that \cref{thm:main-ctw-list-hard} yields the following corollary. (generalize Chudnovsky et al.)

\begin{corollary}
Let $F$ be a fixed connected graph, which is not a path or a subdivided claw.
Let $\mathcal{H}$ be the class of connected non-bi-arc graphs.
\begin{enumerate}[a)]
\item For every $H \in \mathcal{H}$, there is no algorithm that solves every instance $(G,L)$ of  $\lhomo H$, where $G$ is $F$-free, in time $(mim^*(H)-\epsilon)^{\ctw{G}} \cdot |V(G)|^{\Oh(1)}$ for any $\epsilon > 0$, unless the SETH fails,
\item There exists a universal constant $0<\delta<1$, such that for every $H \in \mathcal{H}$, there is no algorithm that solves every instance $(G,L)$ of $\lhomo H$, where $G$ is $F$-free, in time $mim^*(H)^{\delta \cdot \ctw{G}} \cdot |V(G)|^{\Oh(1)}$, unless the ETH fails.
\end{enumerate}
\end{corollary}

$\pw{G} \leq \ctw{G}$

%\begin{corollary}\label{thm:main-pw-deg3}
%Let $H$ be a connected graph (with possible loops), which is not a bi-arc graph, and let $k=mim(H)$. Let $G$ be a graph with $n$ vertices, the pathwidth $s$ and the maximum degree $3$. Assuming the SETH, there is no algorithm that solves $\lhomo H$ for every $G$ and $L$ in time $(k-\epsilon)^{s} \cdot n^{\Oh(1)}$ for any $\epsilon > 0$.
%\end{corollary}\marta{nie wiem czy to ciekawe jest teraz i czy pisać ten wniosek}

We answer a question of Jansen~\cite{BartPersonal}, re-iterated by Okrasa \emph{et al.}~\cite{LhomoTreewidth}.

\begin{restatable}{theorem}{mainctwhomo}
%\begin{theorem}
\label{thm:main-ctw-nonlist-hard}
Let $\mathcal{H}$ be the class of connected non-bipartite projective cores with at least three vertices.
\begin{enumerate}[a)]
\item  For every $H \in \mathcal{H}$, there is no algorithm that solves every instance $G$ of  $\homo H$ in time $(mim^*(H)-\epsilon)^{\ctw{G}} \cdot |V(G)|^{\Oh(1)}$ for any $\epsilon > 0$, unless the SETH fails,

\item There exists a universal constant $0<\delta<1$, such that for every $H \in \mathcal{H}$, there is no algorithm that solves every instance $G$ of $\homo H$ in time $mim^*(H)^{\delta \cdot \ctw{G}} \cdot |V(G)|^{\Oh(1)}$, unless the ETH fails.
\end{enumerate}
%\end{theorem}
\end{restatable}


\begin{restatable}{corollary}{corcyclesctw}
%\begin{corollary}
Let $\mathcal{C}$ be the family of odd cycles.
Then for $C \in \mathcal{C}$, there is no algorithm that solves $\homo{C}$ for instances $G$ in time $2^{o(\log |V(C)| \cdot \ctw{G})} \cdot |V(G)|^{\Oh(1)}$, unless the ETH fails. \newline
In particular, there is no universal constant $c$, such that $\homo{C}$ can be solved in time $c^{\ctw{G}} \cdot |V(G)|^{\Oh(1)}$ for every $C \in \mathcal{C}$ and every instance $G$.
%\end{corollary}
\end{restatable}



In the next theorem $\omega < 2.373$ is the matrix multiplication exponent, see Coppersmith, Winograd~\cite{DBLP:journals/jsc/CoppersmithW90} and Vassilevska-Williams~\cite{DBLP:conf/stoc/Williams12}

\begin{restatable}{corollary}{algolhomo}
%\begin{corollary}
Let $H$ be a graph with possible loops  and let $(G,L)$ is an instance of $\lhomo{H}$, where $G$ is given with a linear layout of width $k$.
Then $(G,L)$ can be solved in time $2^{\gamma^*(H) \cdot \omega \cdot k} \cdot (|V(G)| \cdot |V(H)|)^{\Oh(1)}$.
%\end{corollary}
\end{restatable}



==> reduction-pw3.tex <==
%\begin{proof}[Proof of \cref{thm:bipartite-undecomp}c)]
%Let $\phi$ be an instance of CNF-SAT with $n$ variables and $m$ clauses. Let $S$ be a strongly incomparable set of size $mim(H)$ and let $(G,L)$ be an instance of $\lhomo H$ constructed as in the proof of \cref{thm:bipartite-undecomp}. We will construct an instance $(\widetilde{G},\widetilde{L})$ of $\lhomo H$ such that: maximum degree of $\widetilde{G}$ is $3$, pathwidth of $\widetilde{G}$ is at most $\pw{G}+1$ and $(\widetilde{G},\widetilde{L})\to H$ if and only if $(G,L)\to H$. 
%\end{proof}

Note that the instances constructed in the proofs satisfy conditions 1. and 2. of \cref{def:consist-inst}. Moreover, in any instance of $\lhomo {H}$ we can always remove comparable vertices from the lists. Thus we actually proved the following.

\begin{corollary}\label{cor:consist-hard}
\cref{thm:bipartite} and \cref{cor:ctw-list-eth} hold, even if we assume that the instance $(G,L)$ is constistent.
\end{corollary}

==> upperbound.tex <==
\prz[inline]{ta sekcja wyleci}

\begin{theorem}[\cite{LhomoTreewidth}]\label{thm:treewidth}
Let $H$ be a connected non-bi-arc graph (with possible loops), and let $k=i^*(H)$. Let $G$ be a graph with $n$ vertices, given with a tree decomposition of width $t$. Even if $H$ is given as an input, every instance $(G,L)$ of the $\lhomo{H}$ problem with instance $(G,L)$ can be solved in time $k^{t} \cdot (n\cdot |H|)^{\Oh(1)}$.
\end{theorem}

Let us show that \cref{thm:treewidth} implies \cref{thm:main}~a).

\begin{proof}[Proof of \cref{thm:main}~a)]
By \cref{prop:fvs-tw}, if $G$ is given along with a feedback vertex set of size $s$, then in polynomial time we can construct a tree decompostion of $G$ of width $s+1$. Thus we can use the algorithm given by \cref{thm:treewidth} to decide whether $(G,L) \to H$. The total running time is:
\[
i^*(H)^{s+1} \cdot (n\cdot |H|)^{\Oh(1)}=i^*(H)^{s} \cdot i^*(H) \cdot (n\cdot |H|)^{\Oh(1)}=i^*(H)^{s} \cdot (n\cdot |H|)^{\Oh(1)},
\]
where the last equality follows from the fact that $i^*(H)\leq|H|$.
\end{proof}
